Kruskal's Tree Theorem for Acyclic Term Graphs

In this paper we study termination of term graph rewriting, where we restrict our attention to acyclic term graphs. Motivated by earlier work by Plump we aim at a definition of the notion of simplification order for acyclic term graphs. For this we adapt the homeomorphic embedding relation to term graphs. In contrast to earlier extensions, our notion is inspired by morphisms. Based on this, we establish a variant of Kruskal's Tree Theorem formulated for acyclic term graphs. In proof, we rely on the new notion of embedding and follow Nash-Williams' minimal bad sequence argument. Finally, we propose a variant of the lexicographic path order for acyclic term graphs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{25}
\providecommand{\publicationstatus}{A. Corradini \& H. Zantema (Eds.)\\
Computing with Terms and Graphs (TERMGRAPH 2016)\\
EPTCS 225, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.225.5}{10.4204/EPTCS.225.5}}
\pdfoutput=1

